A 3D radiative transfer framework: VI. PHOENIX/3D example applications

We demonstrate the application of our 3D radiative transfer framework in the model atmosphere code PHOENIX/3D for a number of spectrum synthesis calculations for very different conditions. The 3DRT framework discussed in the previous papers of this series was added to our general-purpose model atmosphere code PHOENIX/1D and an extended 3D version PHOENIX/3D was created. The \phxT code is parallelized via the MPI library using a hierarchical domain decomposition and displays very good strong scaling. We present the results of several test cases for widely different atmosphere conditions and compare the 3D calculations with equivalent 1D models to assess the internal accuracy of the 3D modeling. In addition, we show the results for a number of parameterized 3D structures. With presently available computational resources it is possible to solve the full 3D radiative transfer (including scattering) problem with the same micro-physics as included in 1D modeling.

==> aa.tex <==
%%==================================================================%%
%%                                                                  %%
%%                                                                  %%
%%                                                                  %%
%%                      A S T R O N O M Y                           %%
%%                                                                  %%
%%                           AND                                    %%
%%                                                                  %%
%%                  A S T R O P H Y S I C S                         %%
%%                                                                  %%
%%                                                                  %%
%%   Plain TeX Support                           Version 2.0, 1991  %%
%%                                                                  %%
%%   This is file AA.TEX the short startup file of the macro        %%
%%   package                                                        %%
%%   Version 2.0 as of 25 Feb 1991                                  %%
%%                                                                  %%
%%==================================================================%%
%
\input aa.cmm
%
%  \refereelayout           % a referee layout
%
  \MAINTITLE={ ????? }      % must be given
%
%
% \FOOTNOTE{ ????? }          \FOOTNOTE is valid only in
%                             \MAINTITLE or in \SUBTITLE
%
  \SUBTITLE={ ????? }       % is optional
%
  \AUTHOR={ ????? }         % Firstname Name<@number><, Nextauthor@number>
%                             items in "<  >" are optional
%                             \PRESADD{Present address} is optional
%
  \INSTITUTE={ ????? }      % Take care of the affiliations used with \AUTHOR
%                             @1 Institute No.1<@2 next institute>
%
  \ABSTRACT={ ????? }       % must be given
%
  \KEYWORDS={ ????? }       % must be given
%
  \THESAURUS={ ????? }      % must be given
%
  \OFFPRINTS={ ????? }      % is optional
%
  \DATE={ ????? }           % must be given at the last moment
%
% Please don't overrule this command, it will format your titlepage.
\maketitle
%
% Now start your text using the Springer macros see the
% instructions in file AA.DOC or the examples in AA.DEM
%
\bye                          % finish your text with this command

